The SRG/eROSITA All-Sky Survey. The Weak-Lensing Mass Calibration and the Stellar Mass-to-Halo Mass Relation from the Hyper Suprime-Cam Subaru Strategic Program

We present the weak-lensing mass calibration and constrain the BCG (brightest cluster galaxy) stellar-mass-to-halo-mass-and-redshift ($M_{\star,\mathrm{BCG}}-M-z$) relation for a sample of $124$ galaxy clusters and groups at redshift $0.1<z<0.8$ from the first Data Release of the $eROSITA$ All-Sky Survey (eRASS1), using data from the Hyper Suprime-Cam (HSC) Subaru Strategic Program. The cluster survey is conducted by the $eROSITA$ X-ray telescope aboard the Spectrum-Roentgen-Gamma (SRG) space observatory. The cluster sample is X-ray-selected and optically confirmed with a negligibly low contamination rate ($\approx5%$). On a basis of individual clusters, the shear profiles of $96$ clusters are derived using the HSC Three-Year (HSC-Y3) weak-lensing data, while the BCG stellar masses of $101$ clusters are estimated using the SED template fitting to the HSC five-band ($grizY$) photometry. The observed X-ray photon count rate is used as the mass proxy, based on which individual halo masses are obtained at the given count rate in a population modelling while accounting for systematic uncertainties in the weak-lensing modelling through a simulation-calibrated weak-lensing mass-to-halo-mass relation. The count rate and BCG stellar mass relations are simultaneously constrained in a forward and population modelling. In agreement with the results based on the weak-lensing data from the DES and KiDS surveys, we obtain a count rate relation with a self-similar redshift scaling and a mass trend that is steeper than the self-similar prediction. Our results suggest that the BCG stellar mass at a fixed halo mass has remained stable with a moderate increase at a level of $\left(20\pm8\right)%$ since redshift $z\approx0.8$. This finding supports the picture of the ``rapid-then-slow'' BCG formation, where the majority of the stellar mass must have been assembled at much earlier cosmic time.

==> bcg_images.tex <==
%
\begin{figure*}[!ht]
\centering
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/3_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/4_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/5_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/7_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/12_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/13_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/14_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/23_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/25_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/26_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/27_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/30_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/32_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/33_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/34_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/35_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/36_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/38_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/43_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/44_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/46_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/47_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/49_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/50_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/52_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/53_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/54_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/55_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/56_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/57_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/59_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/60_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/61_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/63_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/65_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/68_rgb.png}}
\caption{See Appendix~\ref{app:imaging} for details.}
\label{fig:cutout1}
\end{figure*}
%
%
\begin{figure*}[!ht]
\centering
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/70_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/71_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/72_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/73_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/74_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/76_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/78_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/79_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/80_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/81_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/82_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/83_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/85_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/86_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/87_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/93_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/94_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/96_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/97_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/99_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/100_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/101_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/102_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/105_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/107_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/108_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/111_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/112_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/116_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/117_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/119_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/120_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/121_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/124_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/125_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/127_rgb.png}}
\caption{See Appendix~\ref{app:imaging} for details.}
\label{fig:cutout2}
\end{figure*}
%
%
\begin{figure*}[!ht]
\centering
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/151_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/154_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/156_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/157_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/160_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/161_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/169_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/171_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/172_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/174_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/176_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/178_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/179_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/181_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/186_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/189_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/190_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/191_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/192_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/194_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/195_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/196_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/197_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/199_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/201_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/202_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/204_rgb.png}}\\
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/207_rgb.png}}
\resizebox{0.33\textwidth}{!}{\includegraphics[scale=1]{pplots/images/208_rgb.png}}
\caption{See Appendix~\ref{app:imaging} for details.}
\label{fig:cutout3}
\end{figure*}
%


==> newcommands.tex <==
% cosmo
\newcommand{\lcdm}{\ensuremath{\Lambda\textrm{CDM}}}
\newcommand{\wcdm}{\ensuremath{w\textrm{CDM}}}
\newcommand{\omegam}{\ensuremath{\Omega_{\mathrm{m}}}}
\newcommand{\omegal}{\ensuremath{\Omega_{\Lambda}}}
\newcommand{\omegab}{\ensuremath{\Omega_{\mathrm{b}}}}
\newcommand{\omegak}{\ensuremath{\Omega_{\mathrm{k}}}}
\newcommand{\Hnow}{\ensuremath{H_{0}}}
\newcommand{\hnow}{\ensuremath{h}}
\newcommand{\h}{\ensuremath{h}}
\newcommand{\sigmaeight}{\ensuremath{\sigma_{8}}}
\newcommand{\seight}{\ensuremath{\hat{S}_{8}}}
\newcommand{\ns}{\ensuremath{n_{\mathrm{s}}}}
\newcommand{\w}{\ensuremath{w}}
% basics
\newcommand{\percent}{\ensuremath{\%}}
\newcommand{\Msun}{\ensuremath{\mathrm{M}_{\odot}}}
\newcommand{\Msunh}{\ensuremath{h^{-1}\mathrm{M}_{\odot}}}
\newcommand{\Mpc}{\ensuremath{\mathrm{Mpc}}}
\newcommand{\Mpch}{\ensuremath{h^{-1}\mathrm{Mpc}}}
\newcommand{\Lsun}{\ensuremath{\mathrm{L}_{\odot}}}
\newcommand{\Rfiveoo}{\ensuremath{R_{500\mathrm{c}}}}
\newcommand{\Mfiveoo}{\ensuremath{M_{500\mathrm{c}}}}
\newcommand{\cfiveoo}{\ensuremath{c_{500\mathrm{c}}}}
\newcommand{\Rtwooo}{\ensuremath{R_{200\mathrm{c}}}}
\newcommand{\Mtwooo}{\ensuremath{M_{200\mathrm{c}}}}
\newcommand{\ctwooo}{\ensuremath{c_{200\mathrm{c}}}}
\newcommand{\redshift}{\ensuremath{z}}
\newcommand{\mass}{\ensuremath{M}}
\newcommand{\dif}{\ensuremath{\mathrm{d}}}
\newcommand{\angstrom}{\textup{\AA}}
\newcommand{\rhocrit}{\ensuremath{\rho_{\mathrm{c}}}}
% instruments or surveys
\newcommand{\chandra}{\emph{Chandra}}
\newcommand{\xmm}{XMM-\emph{Newton}}
\newcommand{\planck}{\emph{Planck}}
\newcommand{\wmap}{\emph{WMAP}}
\newcommand{\erosita}{\emph{eROSITA}}
\newcommand{\efeds}{eFEDS}
\newcommand{\rosat}{\emph{ROSAT}}
\newcommand{\xxl}{\emph{XXL}}
\newcommand{\wise}{\emph{WISE}}
\newcommand{\rass}{RASS}
\newcommand{\erass}{eRASS}
%
\newcommand{\fcont}{\ensuremath{f_{\mathrm{cont}}}}
% lensing measurements
\newcommand{\mbias}{\ensuremath{m_{\gamma}}}
\newcommand{\wl}{\ensuremath{\mathrm{WL}}}
\newcommand{\zcl}{\ensuremath{z_{\mathrm{cl}}}}
\newcommand{\zs}{\ensuremath{z_{\mathrm{s}}}}
\newcommand{\rshear}{\ensuremath{\gamma_{+}}}
\newcommand{\rshearmod}{\ensuremath{\gamma_{+}^{\mathrm{mod}}}}
\newcommand{\gshear}{\ensuremath{g_{+}}}
\newcommand{\gshearmod}{\ensuremath{g_{+}^{\mathrm{mod}}}}
\newcommand{\convergence}{\ensuremath{\kappa}}
\newcommand{\convergencemod}{\ensuremath{\kappa^{\mathrm{mod}}}}
\newcommand{\eplus}{\ensuremath{e_{+}}}
\newcommand{\rcros}{\ensuremath{\gamma_{\times}}}
\newcommand{\gcros}{\ensuremath{g_{\times}}}
\newcommand{\ecros}{\ensuremath{e_{\times}}}
\newcommand{\lensingw}{\ensuremath{w}}
\newcommand{\deltaSigma}{\ensuremath{\Delta{\Sigma}_{\mathrm{m}}}}
\newcommand{\deltaSigmamod}{\ensuremath{\Delta{\Sigma}_{\mathrm{m}}^{\mathrm{mod}}}}
\newcommand{\Sigmam}{\ensuremath{{\Sigma}_{\mathrm{m}}}}
\newcommand{\Sigmammod}{\ensuremath{{\Sigma}_{\mathrm{m}}^{\mathrm{mod}}}}
\newcommand{\Sigmamcen}{\ensuremath{{\Sigma}_{\mathrm{m}}^{\mathrm{cen}}}}
\newcommand{\Sigmammis}{\ensuremath{{\Sigma}_{\mathrm{m}}^{\mathrm{mis}}}}
\newcommand{\bz}{\ensuremath{b_{z}}}
\newcommand{\bwl}{\ensuremath{b_{\mathrm{WL}}}}
\newcommand{\mwl}{\ensuremath{M_{\mathrm{WL}}}}
\newcommand{\sigmacrit}{\ensuremath{\Sigma_{\mathrm{crit}}}}
\newcommand{\lensingeff}{\ensuremath{\beta}}
\newcommand{\rs}{\ensuremath{r_{\mathrm{s}}}}
\newcommand{\rhos}{\ensuremath{\rho_{\mathrm{s}}}}
\newcommand{\snr}{\ensuremath{\nu}}
\newcommand{\numin}{\ensuremath{\nu_{\mathrm{min}}}}
\newcommand{\mkappanohat}{\ensuremath{M_{\kappa}}}
\newcommand{\mkappa}{\ensuremath{\hat{M}_{\kappa}}}
\newcommand{\thetas}{\ensuremath{\theta_{\mathrm{s}}}}
\newcommand{\sigmashape}{\ensuremath{\sigma_{\kappa}}}
\newcommand{\sigmaconcen}{\ensuremath{\sigma_{c}}}
\newcommand{\Ufilter}{\ensuremath{U}}
\newcommand{\Qfilter}{\ensuremath{Q}}
\newcommand{\rdd}{\ensuremath{R}}
\newcommand{\rddd}{\ensuremath{r}}
\newcommand{\comp}{\ensuremath{\mathcal{C}}}
% likelihoods
\newcommand{\Xlabel}{\ensuremath{\mathcal{X}}}
\newcommand{\Deltaz}{\ensuremath{\Delta z}}
% sr parameters
\newcommand{\mpiv}{\ensuremath{M_{\mathrm{piv}}}}
\newcommand{\zpiv}{\ensuremath{z_{\mathrm{piv}}}}
\newcommand{\Ez}{\ensuremath{E(z)}}
\newcommand{\Ezpiv}{\ensuremath{E(z_{\mathrm{piv}})}}
% xray
\newcommand{\lext}{\ensuremath{L_{\mathrm{ext}}}}
\newcommand{\ldet}{\ensuremath{L_{\mathrm{det}}}}
\newcommand{\rate}{\ensuremath{C_{\mathrm{R}}}}
\newcommand{\ratehat}{\ensuremath{\hat{C}_{\mathrm{R}}}}
\newcommand{\Arate}{\ensuremath{A_{\mathrm{X}}}}
\newcommand{\Brate}{\ensuremath{B_{\mathrm{X}}}}
\newcommand{\deltarate}{\ensuremath{\delta_{\mathrm{X}}}}
\newcommand{\gammarate}{\ensuremath{\gamma_{\mathrm{X}}}}
\newcommand{\sigmarate}{\ensuremath{\sigma_{\mathrm{X}}}}
% nir
\newcommand{\wone}{\ensuremath{W_{1}}}
\newcommand{\wtwo}{\ensuremath{W_{2}}}
% WL
\newcommand{\Awl}{\ensuremath{A_{\mathrm{WL}}}}
\newcommand{\Bwl}{\ensuremath{B_{\mathrm{WL}}}}
\newcommand{\deltawl}{\ensuremath{\delta_{\mathrm{WL}}}}
\newcommand{\gammawl}{\ensuremath{\gamma_{\mathrm{WL}}}}
\newcommand{\sigmawl}{\ensuremath{\sigma_{\mathrm{WL}}}}
% richness
\newcommand{\rich}{\ensuremath{\lambda}}
\newcommand{\Arich}{\ensuremath{A_{\lambda}}}
\newcommand{\Brich}{\ensuremath{B_{\lambda}}}
\newcommand{\deltarich}{\ensuremath{\delta_{\lambda}}}
\newcommand{\gammarich}{\ensuremath{\gamma_{\lambda}}}
\newcommand{\sigmarich}{\ensuremath{\sigma_{\lambda}}}
% BCG
\newcommand{\mbcg}{\ensuremath{M_{\star,\mathrm{BCG}}}}
\newcommand{\mbcghat}{\ensuremath{\hat{M}_{\star,\mathrm{BCG}}}}
\newcommand{\Abcg}{\ensuremath{A_{\mathrm{BCG}}}}
\newcommand{\Bbcg}{\ensuremath{B_{\mathrm{BCG}}}}
\newcommand{\deltabcg}{\ensuremath{\delta_{\mathrm{BCG}}}}
\newcommand{\gammabcg}{\ensuremath{\gamma_{\mathrm{BCG}}}}
\newcommand{\sigmabcg}{\ensuremath{\sigma_{\mathrm{BCG}}}}
% correlated scatter
\newcommand{\rhowlxray}{\ensuremath{\rho_{\mathrm{WL},\mathrm{X}}}}
\newcommand{\rhowlmbcg}{\ensuremath{\rho_{\mathrm{WL},M_{\star,\mathrm{BCG}}}}}
\newcommand{\rhombcgxray}{\ensuremath{\rho_{\mathrm{X},M_{\star,\mathrm{BCG}}}}}

==> pplots/measurements.tex <==
 1eRASS~J083652.6$+$030000 & $( 129.21437, 3.00035 )$ & WL & $ 0.19 $ & $ 14.22 \pm 0.13 $ & $ 14.11 $& $ \cdots $ \\
 1eRASS~J083811.9$-$015938 & $( 129.54900, -1.99318 )$ & BCG & $ 0.56 $ & $ 14.66 \pm 0.18 $ & $ 14.44 $& $ 11.28 \pm 0.1113 $ \\
 1eRASS~J083934.2$-$014035 & $( 129.88909, -1.67908 )$ & BCG & $ 0.29 $ & $ 14.51 \pm 0.16 $ & $ 14.61 $& $ 11.57 \pm 0.0722 $ \\
 1eRASS~J084306.7$+$002834 & $( 130.78317, 0.48309 )$ & WL$+$BCG & $ 0.27 $ & $ 14.01 \pm 0.15 $ & $ 14.06 $& $ 11.50 \pm 0.0850 $ \\
 1eRASS~J084342.8$+$040323 & $( 130.92944, 4.05961 )$ & WL & $ 0.21 $ & $ 14.13 \pm 0.15 $ & $ 14.12 $& $ \cdots $ \\
 1eRASS~J084527.7$+$032736 & $( 131.36569, 3.46079 )$ & WL$+$BCG & $ 0.33 $ & $ 14.62 \pm 0.10 $ & $ 14.67 $& $ 11.75 \pm 0.0802 $ \\
 1eRASS~J085029.4$+$001453 & $( 132.61573, 0.25044 )$ & WL & $ 0.20 $ & $ 14.24 \pm 0.13 $ & $ 14.42 $& $ \cdots $ \\
 1eRASS~J085217.5$-$010126 & $( 133.06939, -1.02658 )$ & WL & $ 0.46 $ & $ 14.52 \pm 0.13 $ & $ 14.43 $& $ \cdots $ \\
 1eRASS~J085230.8$+$002509 & $( 133.12620, 0.41976 )$ & WL & $ 0.28 $ & $ 14.27 \pm 0.14 $ & $ 14.08 $& $ \cdots $ \\
 1eRASS~J085435.8$+$003858 & $( 133.65257, 0.64252 )$ & WL$+$BCG & $ 0.11 $ & $ 14.07 \pm 0.13 $ & $ 13.90 $& $ 11.46 \pm 0.0777 $ \\
 1eRASS~J085751.0$+$031014 & $( 134.47521, 3.17645 )$ & WL$+$BCG & $ 0.20 $ & $ 14.49 \pm 0.12 $ & $ 14.50 $& $ 11.02 \pm 0.0665 $ \\
 1eRASS~J085932.4$+$030832 & $( 134.88466, 3.14468 )$ & WL$+$BCG & $ 0.20 $ & $ 14.28 \pm 0.12 $ & $ 14.31 $& $ 11.76 \pm 0.0610 $ \\
 1eRASS~J090131.4$+$030055 & $( 135.37951, 3.01564 )$ & WL & $ 0.20 $ & $ 14.36 \pm 0.13 $ & $ 14.56 $& $ \cdots $ \\
 1eRASS~J090539.7$+$043433 & $( 136.41610, 4.57755 )$ & WL & $ 0.23 $ & $ 14.26 \pm 0.15 $ & $ 14.38 $& $ \cdots $ \\
 1eRASS~J091414.7$+$001922 & $( 138.56511, 0.32408 )$ & WL & $ 0.17 $ & $ 13.97 \pm 0.15 $ & $ 13.99 $& $ \cdots $ \\
 1eRASS~J091453.6$+$041611 & $( 138.71895, 4.26534 )$ & WL & $ 0.14 $ & $ 14.09 \pm 0.14 $ & $ 14.04 $& $ \cdots $ \\
 1eRASS~J091608.3$-$002355 & $( 139.03845, -0.40456 )$ & WL$+$BCG & $ 0.33 $ & $ 14.62 \pm 0.10 $ & $ 14.57 $& $ 11.70 \pm 0.0821 $ \\
 1eRASS~J092050.7$+$024512 & $( 140.20707, 2.75389 )$ & WL$+$BCG & $ 0.28 $ & $ 14.40 \pm 0.11 $ & $ 14.41 $& $ 11.38 \pm 0.0517 $ \\
 1eRASS~J092121.0$+$031735 & $( 140.33795, 3.28701 )$ & WL$+$BCG & $ 0.35 $ & $ 14.67 \pm 0.11 $ & $ 14.66 $& $ 11.89 \pm 0.0743 $ \\
 1eRASS~J092210.0$+$034626 & $( 140.53185, 3.76631 )$ & WL$+$BCG & $ 0.28 $ & $ 14.53 \pm 0.11 $ & $ 14.67 $& $ 11.62 \pm 0.0787 $ \\
 1eRASS~J092546.2$-$014321 & $( 141.43867, -1.72877 )$ & BCG & $ 0.23 $ & $ 14.10 \pm 0.20 $ & $ 14.11 $& $ 11.26 \pm 0.0735 $ \\
 1eRASS~J093025.3$+$021707 & $( 142.60267, 2.29030 )$ & WL$+$BCG & $ 0.54 $ & $ 14.61 \pm 0.13 $ & $ 14.68 $& $ 11.34 \pm 0.1110 $ \\
 1eRASS~J093150.9$-$002220 & $( 142.96262, -0.37049 )$ & WL$+$BCG & $ 0.35 $ & $ 14.39 \pm 0.12 $ & $ 14.50 $& $ 11.87 \pm 0.0884 $ \\
 1eRASS~J093459.9$+$005438 & $( 143.75282, 0.90407 )$ & WL$+$BCG & $ 0.38 $ & $ 14.52 \pm 0.11 $ & $ 14.43 $& $ 11.59 \pm 0.1221 $ \\
 1eRASS~J093512.7$+$004735 & $( 143.80125, 0.82562 )$ & WL$+$BCG & $ 0.36 $ & $ 14.78 \pm 0.09 $ & $ 14.73 $& $ 11.48 \pm 0.0487 $ \\
 1eRASS~J093521.3$+$023222 & $( 143.83756, 2.54326 )$ & WL$+$BCG & $ 0.50 $ & $ 14.71 \pm 0.14 $ & $ 14.82 $& $ 11.54 \pm 0.0727 $ \\
 1eRASS~J093831.3$-$012524 & $( 144.62560, -1.42579 )$ & WL & $ 0.41 $ & $ 14.25 \pm 0.16 $ & $ 13.77 $& $ \cdots $ \\
 1eRASS~J094023.3$+$022824 & $( 145.10245, 2.47763 )$ & WL$+$BCG & $ 0.15 $ & $ 14.48 \pm 0.10 $ & $ 14.60 $& $ 11.41 \pm 0.0700 $ \\
 1eRASS~J094611.9$+$022201 & $( 146.54988, 2.36884 )$ & WL & $ 0.12 $ & $ 14.10 \pm 0.13 $ & $ 14.11 $& $ \cdots $ \\
 1eRASS~J094844.3$+$020019 & $( 147.17811, 2.01425 )$ & WL & $ 0.49 $ & $ 14.54 \pm 0.13 $ & $ 14.50 $& $ \cdots $ \\
 1eRASS~J095341.6$+$014200 & $( 148.42250, 1.70030 )$ & WL & $ 0.11 $ & $ 14.04 \pm 0.14 $ & $ 14.15 $& $ \cdots $ \\
 1eRASS~J095728.1$+$033954 & $( 149.36589, 3.66553 )$ & BCG & $ 0.16 $ & $ 14.11 \pm 0.19 $ & $ 14.03 $& $ 11.32 \pm 0.0753 $ \\
 1eRASS~J095736.6$+$023430 & $( 149.40426, 2.57383 )$ & WL$+$BCG & $ 0.38 $ & $ 14.48 \pm 0.12 $ & $ 14.63 $& $ 12.03 \pm 0.0818 $ \\
 1eRASS~J095759.2$+$032732 & $( 149.49721, 3.45722 )$ & WL & $ 0.16 $ & $ 14.27 \pm 0.13 $ & $ 14.22 $& $ \cdots $ \\
 1eRASS~J095858.4$-$001323 & $( 149.74577, -0.20602 )$ & WL$+$BCG & $ 0.17 $ & $ 14.07 \pm 0.15 $ & $ 13.94 $& $ 11.70 \pm 0.0894 $ \\
 1eRASS~J100023.4$+$044406 & $( 150.09319, 4.73525 )$ & BCG & $ 0.36 $ & $ 14.61 \pm 0.16 $ & $ 14.63 $& $ 11.45 \pm 0.1125 $ \\
 1eRASS~J100502.4$+$045249 & $( 151.26224, 4.87969 )$ & BCG & $ 0.45 $ & $ 14.54 \pm 0.16 $ & $ 14.51 $& $ 11.48 \pm 0.1212 $ \\
 1eRASS~J101231.5$+$023933 & $( 153.13326, 2.65806 )$ & BCG & $ 0.24 $ & $ 14.43 \pm 0.17 $ & $ 14.36 $& $ 11.34 \pm 0.0497 $ \\
 1eRASS~J101536.3$+$023411 & $( 153.90268, 2.56672 )$ & BCG & $ 0.29 $ & $ 14.30 \pm 0.18 $ & $ 13.91 $& $ 11.70 \pm 0.0926 $ \\
 1eRASS~J101846.9$-$013110 & $( 154.69095, -1.51743 )$ & WL$+$BCG & $ 0.39 $ & $ 14.64 \pm 0.12 $ & $ 14.44 $& $ 11.82 \pm 0.0072 $ \\
 1eRASS~J101851.0$-$010105 & $( 154.71202, -1.01761 )$ & WL$+$BCG & $ 0.11 $ & $ 13.85 \pm 0.18 $ & $ 14.13 $& $ 11.28 \pm 0.0791 $ \\
 1eRASS~J102250.3$-$000309 & $( 155.70726, -0.05382 )$ & WL$+$BCG & $ 0.30 $ & $ 14.07 \pm 0.17 $ & $ 14.23 $& $ 10.97 \pm 0.0922 $ \\
 1eRASS~J102310.1$+$022157 & $( 155.79244, 2.36822 )$ & BCG & $ 0.19 $ & $ 14.32 \pm 0.18 $ & $ 14.52 $& $ 11.84 \pm 0.0492 $ \\
 1eRASS~J102339.7$+$041108 & $( 155.91508, 4.18628 )$ & BCG & $ 0.29 $ & $ 14.95 \pm 0.18 $ & $ 14.82 $& $ 11.44 \pm 0.0568 $ \\
 1eRASS~J103450.9$+$042431 & $( 158.70247, 4.40556 )$ & BCG & $ 0.16 $ & $ 14.17 \pm 0.19 $ & $ 14.27 $& $ 11.76 \pm 0.0499 $ \\
 1eRASS~J104003.4$+$015948 & $( 160.02298, 1.98560 )$ & BCG & $ 0.39 $ & $ 14.33 \pm 0.20 $ & $ 14.29 $& $ 11.48 \pm 0.0661 $ \\
 1eRASS~J104723.6$-$010449 & $( 161.84752, -1.07442 )$ & BCG & $ 0.47 $ & $ 14.65 \pm 0.16 $ & $ 14.65 $& $ 11.59 \pm 0.0929 $ \\
 1eRASS~J105039.5$+$001707 & $( 162.66629, 0.28534 )$ & WL$+$BCG & $ 0.60 $ & $ 14.77 \pm 0.12 $ & $ 14.70 $& $ 12.12 \pm 0.0320 $ \\
 1eRASS~J111111.5$+$004454 & $( 167.79674, 0.75210 )$ & WL$+$BCG & $ 0.19 $ & $ 14.35 \pm 0.11 $ & $ 14.19 $& $ 11.52 \pm 0.0738 $ \\
 1eRASS~J111552.0$+$012954 & $( 168.96630, 1.49861 )$ & BCG & $ 0.36 $ & $ 14.87 \pm 0.18 $ & $ 14.95 $& $ 11.37 \pm 0.1269 $ \\
 1eRASS~J112626.5$+$003625 & $( 171.61081, 0.60571 )$ & WL$+$BCG & $ 0.31 $ & $ 14.08 \pm 0.16 $ & $ 14.13 $& $ 11.59 \pm 0.0669 $ \\
 1eRASS~J112818.3$-$005859 & $( 172.07373, -0.98338 )$ & WL$+$BCG & $ 0.46 $ & $ 14.62 \pm 0.11 $ & $ 14.44 $& $ 11.73 \pm 0.3267 $ \\
 1eRASS~J112949.4$+$025546 & $( 172.46347, 2.93823 )$ & BCG & $ 0.24 $ & $ 14.43 \pm 0.17 $ & $ 14.47 $& $ 11.68 \pm 0.0650 $ \\
 1eRASS~J113655.7$+$000612 & $( 174.22743, 0.09299 )$ & WL$+$BCG & $ 0.59 $ & $ 14.74 \pm 0.12 $ & $ 14.85 $& $ 11.74 \pm 0.1017 $ \\
 1eRASS~J113843.1$+$031510 & $( 174.68360, 3.26052 )$ & WL$+$BCG & $ 0.14 $ & $ 13.91 \pm 0.18 $ & $ 13.87 $& $ 11.08 \pm 0.0731 $ \\
 1eRASS~J114341.5$-$014429 & $( 175.87352, -1.74169 )$ & WL & $ 0.12 $ & $ 14.15 \pm 0.17 $ & $ 14.28 $& $ \cdots $ \\
 1eRASS~J114441.9$+$004414 & $( 176.17379, 0.73734 )$ & WL$+$BCG & $ 0.33 $ & $ 14.35 \pm 0.12 $ & $ 14.23 $& $ 11.47 \pm 0.1185 $ \\
 1eRASS~J114647.4$-$012428 & $( 176.69839, -1.41111 )$ & WL & $ 0.33 $ & $ 14.08 \pm 0.17 $ & $ 13.99 $& $ \cdots $ \\
 1eRASS~J115019.2$-$003637 & $( 177.58504, -0.59318 )$ & WL$+$BCG & $ 0.14 $ & $ 14.06 \pm 0.13 $ & $ 14.02 $& $ 11.12 \pm 0.0651 $ \\
 1eRASS~J115208.5$-$004726 & $( 178.02708, -0.78046 )$ & WL$+$BCG & $ 0.26 $ & $ 13.41 \pm 0.29 $ & $ 13.33 $& $ 11.13 \pm 0.0274 $ \\
 1eRASS~J115214.5$+$003057 & $( 178.05915, 0.52395 )$ & WL$+$BCG & $ 0.47 $ & $ 14.45 \pm 0.13 $ & $ 14.54 $& $ 11.37 \pm 0.0492 $ \\
 1eRASS~J115235.7$+$035642 & $( 178.14592, 3.93986 )$ & WL$+$BCG & $ 0.68 $ & $ 14.53 \pm 0.16 $ & $ 14.59 $& $ 11.23 \pm 0.1730 $ \\
 1eRASS~J115417.0$+$022123 & $( 178.57200, 2.35657 )$ & WL$+$BCG & $ 0.74 $ & $ 14.64 \pm 0.16 $ & $ 14.64 $& $ 11.86 \pm 0.1339 $ \\
 1eRASS~J115620.0$-$001220 & $( 179.08350, -0.20553 )$ & WL$+$BCG & $ 0.11 $ & $ 14.03 \pm 0.13 $ & $ 13.98 $& $ 11.47 \pm 0.0750 $ \\
 1eRASS~J120024.4$+$032112 & $( 180.10549, 3.34696 )$ & WL$+$BCG & $ 0.14 $ & $ 14.71 \pm 0.10 $ & $ 14.89 $& $ 11.55 \pm 0.0848 $ \\
 1eRASS~J120143.7$-$001110 & $( 180.43196, -0.18456 )$ & WL$+$BCG & $ 0.17 $ & $ 14.41 \pm 0.11 $ & $ 14.46 $& $ 11.10 \pm 0.0721 $ \\
 1eRASS~J120358.5$+$012624 & $( 180.99168, 1.42579 )$ & WL$+$BCG & $ 0.39 $ & $ 14.64 \pm 0.12 $ & $ 14.55 $& $ 11.81 \pm 0.0750 $ \\
 1eRASS~J120417.3$+$025402 & $( 181.07295, 2.89815 )$ & WL & $ 0.15 $ & $ 14.06 \pm 0.14 $ & $ 14.08 $& $ \cdots $ \\
 1eRASS~J120954.5$-$003328 & $( 182.47791, -0.55770 )$ & WL$+$BCG & $ 0.18 $ & $ 14.09 \pm 0.14 $ & $ 14.17 $& $ 11.70 \pm 0.0629 $ \\
 1eRASS~J121016.3$+$022338 & $( 182.57381, 2.39546 )$ & WL$+$BCG & $ 0.38 $ & $ 14.56 \pm 0.13 $ & $ 14.62 $& $ 12.04 \pm 0.0051 $ \\
 1eRASS~J121336.5$+$025331 & $( 183.39372, 2.89887 )$ & WL & $ 0.39 $ & $ 14.32 \pm 0.13 $ & $ 14.14 $& $ \cdots $ \\
 1eRASS~J121503.9$-$012741 & $( 183.77197, -1.46098 )$ & WL$+$BCG & $ 0.20 $ & $ 14.22 \pm 0.15 $ & $ 14.23 $& $ 11.66 \pm 0.0405 $ \\
 1eRASS~J122226.1$-$012659 & $( 185.61026, -1.45326 )$ & WL$+$BCG & $ 0.28 $ & $ 14.36 \pm 0.13 $ & $ 14.58 $& $ 11.37 \pm 0.0836 $ \\
 1eRASS~J122242.4$-$013029 & $( 185.67767, -1.51167 )$ & WL$+$BCG & $ 0.29 $ & $ 14.36 \pm 0.14 $ & $ 14.53 $& $ 11.46 \pm 0.0829 $ \\
 1eRASS~J122420.6$+$021206 & $( 186.09158, 2.20303 )$ & WL$+$BCG & $ 0.45 $ & $ 14.62 \pm 0.12 $ & $ 14.62 $& $ 12.11 \pm 0.1678 $ \\
 1eRASS~J122528.9$+$004237 & $( 186.36363, 0.71004 )$ & WL$+$BCG & $ 0.24 $ & $ 14.08 \pm 0.16 $ & $ 14.13 $& $ 11.51 \pm 0.0758 $ \\
 1eRASS~J122644.5$-$003724 & $( 186.68702, -0.62162 )$ & WL$+$BCG & $ 0.16 $ & $ 13.98 \pm 0.15 $ & $ 13.81 $& $ 11.34 \pm 0.0754 $ \\
 1eRASS~J123055.0$+$024716 & $( 187.72970, 2.78710 )$ & BCG & $ 0.39 $ & $ 14.57 \pm 0.16 $ & $ 14.65 $& $ 11.49 \pm 0.1543 $ \\
 1eRASS~J123108.4$+$003653 & $( 187.78493, 0.61363 )$ & WL & $ 0.47 $ & $ 14.45 \pm 0.16 $ & $ 14.33 $& $ \cdots $ \\
 1eRASS~J123740.7$-$012119 & $( 189.42311, -1.36062 )$ & WL$+$BCG & $ 0.16 $ & $ 14.13 \pm 0.15 $ & $ 14.18 $& $ 11.88 \pm 0.0702 $ \\
 1eRASS~J123755.2$-$001611 & $( 189.48058, -0.27471 )$ & WL$+$BCG & $ 0.14 $ & $ 13.98 \pm 0.14 $ & $ 14.03 $& $ 11.20 \pm 0.0730 $ \\
 1eRASS~J124503.8$-$002823 & $( 191.28558, -0.46177 )$ & WL & $ 0.23 $ & $ 14.00 \pm 0.16 $ & $ 14.14 $& $ \cdots $ \\
 1eRASS~J124942.4$+$014447 & $( 192.43193, 1.74645 )$ & BCG & $ 0.20 $ & $ 14.09 \pm 0.20 $ & $ 14.15 $& $ 11.59 \pm 0.0818 $ \\
 1eRASS~J125035.8$+$003646 & $( 192.64934, 0.61281 )$ & WL$+$BCG & $ 0.63 $ & $ 14.54 \pm 0.14 $ & $ 14.23 $& $ 11.83 \pm 0.0398 $ \\
 1eRASS~J125728.4$+$011841 & $( 194.37388, 1.31586 )$ & BCG & $ 0.37 $ & $ 14.19 \pm 0.19 $ & $ 13.75 $& $ 11.35 \pm 0.0685 $ \\
 1eRASS~J130037.3$-$015635 & $( 195.15752, -1.94352 )$ & BCG & $ 0.44 $ & $ 14.39 \pm 0.17 $ & $ 14.27 $& $ 11.73 \pm 0.1211 $ \\
 1eRASS~J130709.0$+$011222 & $( 196.77408, 1.20512 )$ & WL$+$BCG & $ 0.19 $ & $ 13.95 \pm 0.18 $ & $ 14.13 $& $ 11.31 \pm 0.0666 $ \\
 1eRASS~J131129.4$-$012026 & $( 197.87297, -1.34109 )$ & WL$+$BCG & $ 0.18 $ & $ 14.98 \pm 0.11 $ & $ 15.01 $& $ 11.24 \pm 0.0561 $ \\
 1eRASS~J131419.1$-$012723 & $( 198.58215, -1.45715 )$ & WL$+$BCG & $ 0.18 $ & $ 14.13 \pm 0.15 $ & $ 13.81 $& $ 11.73 \pm 0.0762 $ \\
 1eRASS~J131814.0$+$014253 & $( 199.55881, 1.71313 )$ & BCG & $ 0.23 $ & $ 14.05 \pm 0.20 $ & $ 14.18 $& $ 11.36 \pm 0.0761 $ \\
 1eRASS~J131815.6$-$003818 & $( 199.55704, -0.62596 )$ & WL$+$BCG & $ 0.10 $ & $ 13.63 \pm 0.22 $ & $ 13.67 $& $ 11.52 \pm 0.0776 $ \\
 1eRASS~J131815.3$-$011004 & $( 199.56356, -1.16890 )$ & WL & $ 0.22 $ & $ 14.29 \pm 0.18 $ & $ 14.18 $& $ \cdots $ \\
 1eRASS~J131823.9$-$003135 & $( 199.59810, -0.52953 )$ & WL$+$BCG & $ 0.11 $ & $ 13.76 \pm 0.20 $ & $ 13.96 $& $ 11.60 \pm 0.0573 $ \\
 1eRASS~J134304.9$-$000053 & $( 205.76907, -0.01546 )$ & BCG & $ 0.68 $ & $ 14.50 \pm 0.17 $ & $ 14.56 $& $ 11.60 \pm 0.1429 $ \\
 1eRASS~J134525.0$+$001207 & $( 206.34472, 0.20605 )$ & WL$+$BCG & $ 0.25 $ & $ 14.14 \pm 0.15 $ & $ 14.41 $& $ 11.48 \pm 0.0760 $ \\
 1eRASS~J134745.7$+$012441 & $( 206.94083, 1.41249 )$ & BCG & $ 0.57 $ & $ 14.53 \pm 0.16 $ & $ 14.30 $& $ 11.86 \pm 0.1267 $ \\
 1eRASS~J134840.1$+$003907 & $( 207.17319, 0.65456 )$ & WL$+$BCG & $ 0.42 $ & $ 14.33 \pm 0.14 $ & $ 14.34 $& $ 12.07 \pm 0.0624 $ \\
 1eRASS~J135326.5$+$000255 & $( 208.35942, 0.04664 )$ & WL$+$BCG & $ 0.11 $ & $ 13.93 \pm 0.16 $ & $ 14.04 $& $ 11.19 \pm 0.0841 $ \\
 1eRASS~J135424.2$-$010250 & $( 208.60017, -1.04431 )$ & WL$+$BCG & $ 0.15 $ & $ 14.40 \pm 0.11 $ & $ 14.37 $& $ 11.78 \pm 0.0725 $ \\
 1eRASS~J140559.3$+$013843 & $( 211.49715, 1.64785 )$ & BCG & $ 0.17 $ & $ 13.93 \pm 0.20 $ & $ 13.15 $& $ 11.17 \pm 0.0618 $ \\
 1eRASS~J140707.1$-$001450 & $( 211.77931, -0.25140 )$ & WL$+$BCG & $ 0.55 $ & $ 14.64 \pm 0.13 $ & $ 14.57 $& $ 11.85 \pm 0.0320 $ \\
 1eRASS~J140959.6$-$013230 & $( 212.49782, -1.53965 )$ & WL$+$BCG & $ 0.11 $ & $ 13.81 \pm 0.19 $ & $ 14.05 $& $ 11.46 \pm 0.0743 $ \\
 1eRASS~J141055.8$+$013800 & $( 212.73264, 1.63343 )$ & BCG & $ 0.18 $ & $ 14.09 \pm 0.18 $ & $ 14.24 $& $ 11.51 \pm 0.0710 $ \\
 1eRASS~J141452.4$+$001316 & $( 213.73578, 0.20639 )$ & WL$+$BCG & $ 0.12 $ & $ 13.69 \pm 0.17 $ & $ 13.70 $& $ 11.42 \pm 0.0731 $ \\
 1eRASS~J141457.8$-$002050 & $( 213.74060, -0.34965 )$ & WL & $ 0.13 $ & $ 14.51 \pm 0.12 $ & $ 14.46 $& $ \cdots $ \\
 1eRASS~J141507.1$-$002905 & $( 213.78498, -0.49333 )$ & WL$+$BCG & $ 0.13 $ & $ 14.31 \pm 0.12 $ & $ 14.08 $& $ 11.70 \pm 0.0776 $ \\
 1eRASS~J141547.1$+$001530 & $( 213.95354, 0.26047 )$ & WL$+$BCG & $ 0.13 $ & $ 14.02 \pm 0.15 $ & $ 14.08 $& $ 11.02 \pm 0.0818 $ \\
 1eRASS~J142016.3$+$005716 & $( 215.06934, 0.95531 )$ & WL$+$BCG & $ 0.50 $ & $ 14.55 \pm 0.11 $ & $ 14.63 $& $ 11.66 \pm 0.0759 $ \\
 1eRASS~J142724.6$-$001509 & $( 216.85038, -0.24871 )$ & WL$+$BCG & $ 0.16 $ & $ 13.95 \pm 0.14 $ & $ 13.99 $& $ 11.66 \pm 0.0682 $ \\
 1eRASS~J143044.6$+$004815 & $( 217.67543, 0.81749 )$ & WL$+$BCG & $ 0.31 $ & $ 14.37 \pm 0.11 $ & $ 14.36 $& $ 11.45 \pm 0.0692 $ \\
 1eRASS~J143121.5$-$005336 & $( 217.83829, -0.89570 )$ & WL$+$BCG & $ 0.40 $ & $ 14.51 \pm 0.12 $ & $ 14.55 $& $ 11.56 \pm 0.1208 $ \\
 1eRASS~J143736.1$-$001740 & $( 219.43256, -0.31583 )$ & WL$+$BCG & $ 0.14 $ & $ 14.24 \pm 0.12 $ & $ 14.09 $& $ 10.89 \pm 0.0800 $ \\
 1eRASS~J143821.9$+$034012 & $( 219.59115, 3.67036 )$ & BCG & $ 0.22 $ & $ 14.53 \pm 0.17 $ & $ 14.65 $& $ 11.89 \pm 0.0828 $ \\
 1eRASS~J144016.1$+$034155 & $( 220.06095, 3.69504 )$ & BCG & $ 0.28 $ & $ 14.36 \pm 0.17 $ & $ 14.26 $& $ 11.64 \pm 0.0653 $ \\
 1eRASS~J144031.3$-$013738 & $( 220.13343, -1.62420 )$ & WL$+$BCG & $ 0.32 $ & $ 14.57 \pm 0.15 $ & $ 14.48 $& $ 11.16 \pm 0.0481 $ \\
 1eRASS~J144050.2$+$004103 & $( 220.20374, 0.67232 )$ & WL$+$BCG & $ 0.54 $ & $ 14.22 \pm 0.19 $ & $ 14.52 $& $ 11.35 \pm 0.1599 $ \\
 1eRASS~J144133.6$-$005418 & $( 220.38605, -0.89954 )$ & WL$+$BCG & $ 0.54 $ & $ 14.56 \pm 0.13 $ & $ 14.67 $& $ 12.15 \pm 0.0625 $ \\
 1eRASS~J144309.6$+$010214 & $( 220.78878, 1.03670 )$ & WL$+$BCG & $ 0.53 $ & $ 14.57 \pm 0.13 $ & $ 14.59 $& $ 11.99 \pm 0.0655 $ \\
 1eRASS~J144914.3$+$032949 & $( 222.32834, 3.51829 )$ & BCG & $ 0.21 $ & $ 13.89 \pm 0.28 $ & $ 13.91 $& $ 11.07 \pm 0.0782 $ \\
 1eRASS~J144950.6$+$005558 & $( 222.46120, 0.92683 )$ & WL$+$BCG & $ 0.41 $ & $ 14.36 \pm 0.13 $ & $ 14.30 $& $ 11.61 \pm 0.0643 $ \\
 1eRASS~J145004.7$+$004931 & $( 222.52202, 0.82471 )$ & WL & $ 0.38 $ & $ 14.33 \pm 0.13 $ & $ 14.29 $& $ \cdots $ \\
 1eRASS~J145218.8$+$001002 & $( 223.07861, 0.16244 )$ & WL$+$BCG & $ 0.59 $ & $ 14.73 \pm 0.13 $ & $ 15.01 $& $ 11.67 \pm 0.0568 $ \\
 1eRASS~J145459.3$-$011455 & $( 223.74723, -1.24914 )$ & WL$+$BCG & $ 0.31 $ & $ 14.22 \pm 0.14 $ & $ 14.13 $& $ 11.48 \pm 0.0750 $ \\
 1eRASS~J145723.4$+$030717 & $( 224.35304, 3.11794 )$ & BCG & $ 0.63 $ & $ 14.45 \pm 0.17 $ & $ 14.74 $& $ 11.81 \pm 0.0181 $ \\
\hline

==> pplots/posteriors.tex <==
 WL only & $  0.093^{+0.029}_{-0.036} $ & $  1.50^{+0.20}_{-0.30} $ & $  0.7\pm 1.5 $ & $  -0.8^{+1.5}_{-1.1} $ & $  0.56^{+0.17}_{-0.23} $ & $ \cdots $ & $ \cdots $ & $ \cdots $ & $ \cdots $ & $ \cdots $ \\[3pt]
 WL only + $M_{\star,\mathrm{BCG}}$ & $  0.093^{+0.029}_{-0.035} $ & $  1.53^{+0.22}_{-0.30} $ & $  0.8\pm 1.5 $ & $  -0.9^{+1.5}_{-1.1} $ & $  0.56^{+0.16}_{-0.22} $ & $  11.547^{+0.083}_{-0.074} $ & $  0.184^{+0.068}_{-0.16} $ & $  0.22\pm 0.29 $ & $  1.49^{+0.88}_{-0.75} $ & $  0.554^{+0.040}_{-0.049} $ \\[3pt]
 WL only + $M_{\star,\mathrm{BCG}}$ (priors on $\gamma_{\mathrm{BCG}}$) & $  0.084^{+0.025}_{-0.032} $ & $  1.66^{+0.25}_{-0.29} $ & $  1.4^{+1.7}_{-1.5} $ & $  -1.5^{+1.5}_{-1.2} $ & $  0.54^{+0.15}_{-0.20} $ & $  11.433^{+0.066}_{-0.055} $ & $  0.38\pm 0.11 $ & $  0.62\pm 0.25 $ & $  -0.36\pm 0.13 $ & $  0.560^{+0.044}_{-0.055} $ \\[3pt]
\hline

==> pplots/resultcommands.tex <==
\newcommand{\asobs}{\ensuremath{  0.093^{+0.029}_{-0.036} }}
\newcommand{\bsobs}{\ensuremath{  1.50^{+0.20}_{-0.30} }}
\newcommand{\deltasobs}{\ensuremath{  0.7\pm 1.5 }}
\newcommand{\gammasobs}{\ensuremath{  -0.8^{+1.5}_{-1.1} }}
\newcommand{\sigmasobs}{\ensuremath{  0.56^{+0.17}_{-0.23} }}
%
\newcommand{\rhowlsobswlonly}{\ensuremath{  -0.05^{+0.45}_{-0.63} }}
%
\newcommand{\asobswlxo}{\ensuremath{  0.093^{+0.029}_{-0.035} }}
\newcommand{\bsobswlxo}{\ensuremath{  1.53^{+0.22}_{-0.30} }}
\newcommand{\deltasobswlxo}{\ensuremath{  0.8\pm 1.5 }}
\newcommand{\gammasobswlxo}{\ensuremath{  -0.9^{+1.5}_{-1.1} }}
\newcommand{\sigmasobswlxo}{\ensuremath{  0.56^{+0.16}_{-0.22} }}
%
\newcommand{\axobs}{\ensuremath{  11.547^{+0.083}_{-0.074} }}
\newcommand{\bxobs}{\ensuremath{  0.184^{+0.068}_{-0.16} }}
\newcommand{\deltaxobs}{\ensuremath{  0.22\pm 0.29 }}
\newcommand{\gammaxobs}{\ensuremath{  1.49^{+0.88}_{-0.75} }}
\newcommand{\sigmaxobs}{\ensuremath{  0.554^{+0.040}_{-0.049} }}
%
\newcommand{\rhowlsobswlxo}{\ensuremath{  -0.04\pm 0.43 }}
\newcommand{\rhowlxobswlxo}{\ensuremath{  -0.32^{+0.23}_{-0.49} }}
\newcommand{\rhoxobssobswlxo}{\ensuremath{  -0.10^{+0.24}_{-0.27} }}
%
\newcommand{\axobsprioronz}{\ensuremath{  11.433^{+0.066}_{-0.055} }}
\newcommand{\bxobsprioronz}{\ensuremath{  0.38\pm 0.11 }}
\newcommand{\deltaxobsprioronz}{\ensuremath{  0.62\pm 0.25 }}
\newcommand{\gammaxobsprioronz}{\ensuremath{  -0.36\pm 0.13 }}
\newcommand{\sigmaxobsprioronz}{\ensuremath{  0.560^{+0.044}_{-0.055} }}
%
\newcommand{\axobsfulllib}{\ensuremath{  11.498\pm 0.085 }}
\newcommand{\bxobsfulllib}{\ensuremath{  0.192^{+0.057}_{-0.18} }}
\newcommand{\deltaxobsfulllib}{\ensuremath{  0.37^{+0.29}_{-0.32} }}
\newcommand{\gammaxobsfulllib}{\ensuremath{  0.91^{+0.97}_{-0.77} }}
\newcommand{\sigmaxobsfulllib}{\ensuremath{  0.566^{+0.043}_{-0.051} }}
%

